Depth Reconstruction from Sparse Samples: Representation, Algorithm, and Sampling

The rapid development of 3D technology and computer vision applications have motivated a thrust of methodologies for depth acquisition and estimation. However, most existing hardware and software methods have limited performance due to poor depth precision, low resolution and high computational cost. In this paper, we present a computationally efficient method to recover dense depth maps from sparse measurements. We make three contributions. First, we provide empirical evidence that depth maps can be encoded much more sparsely than natural images by using common dictionaries such as wavelets and contourlets. We also show that a combined wavelet-contourlet dictionary achieves better performance than using either dictionary alone. Second, we propose an alternating direction method of multipliers (ADMM) to achieve fast reconstruction. A multi-scale warm start procedure is proposed to speed up the convergence. Third, we propose a two-stage randomized sampling scheme to optimally choose the sampling locations, thus maximizing the reconstruction performance for any given sampling budget. Experimental results show that the proposed method produces high quality dense depth estimates, and is robust to noisy measurements. Applications to real data in stereo matching are demonstrated.

==> customFigureMacros.tex <==
% ===========================================================
% Definitions, commands and environnments for drawing figures
%
% Vivek Goyal
% based on work by
% Ivana Jovanovic, Patrick Vandewalle, Olivier Roy - 2005
% ===========================================================

% --------
% PACKAGES
% --------
%\RequirePackage{amsmath}
%\RequirePackage{amssymb}
\RequirePackage{xspace}
\RequirePackage{bbm}
\RequirePackage{ifthen}
%\RequirePackage{pstricks}
%\RequirePackage{pst-plot}
%\RequirePackage{algo}
%\RequirePackage{epsfig}
%\RequirePackage{latexsym}
%\RequirePackage{subfigure}

% --------------------
% PSTRICKS DEFINITIONS
% --------------------
% Upsampling operation (reference point at the center of the circle)
% Parameter #1: upsampling factor
\def\upsampling#1{

    \pscircle(0,0){0.5}
    \psline{->}(-0.15,-0.25)(-0.15,0.25)
    \rput(0.15,0){#1}

}

% Downsampling operation (reference point at the center of the circle)
% Parameter #1: downsampling factor
\def\downsampling#1{

    \pscircle(0,0){0.5}
    \psline{<-}(-0.15,-0.25)(-0.15,0.25)
    \rput(0.15,0){#1}

}

% Sampling operation (reference point at the center of the box)
% Parameter #1: sampling period
% This is a quick-and-dirty job; definitely less beautiful than other macros.
\def\sampler#1{

    \psframe(-1,-0.5)(1,0.5)
    \psline{-}(-0.6,-0.2)(-0.2,-0.2)
    \psline{-}(0.2,-0.2)(0.6,-0.2)
    \psline{-}(-0.2,-0.2)(0.1,0.1)
    \rput(-0.3,0.3){#1}

}

% Discrete-to-continuous operation (reference point at the center of the box)
% (Generation of weighted Dirac train)
% Parameter #1: sampling period
% This is a quick-and-dirty job; definitely less beautiful than other macros.
\def\diracTrain#1{

    \psframe(-1,-0.5)(1,0.5)
    \psline{-}(-0.8,0)(0.8,0)
    \psline{->}(-0.6,0)(-0.6,-0.45)
    \psline{->}(-0.3,0)(-0.3,-0.3)
    \psline{->}( 0.0,0)( 0.0, 0.4)
    \psline{->}( 0.3,0)( 0.3, 0.4)
    \psline{->}( 0.6,0)( 0.6,-0.35)
    \rput(0.3,-0.2){#1}

}

% Filter (reference point at the center of the box)
% Parameter #1: filter label
\def\filter#1{

    \psframe(-1,-0.5)(1,0.5)
    \rput(0,0){#1}

}

\def\shortfilter#1{

    \psframe(-0.75,-0.5)(0.75,0.5)
    \rput(0,0){#1}

}

% Filter (reference point at the center of the box)
% Parameter #1: filter label
\def\widefilter#1{

    \psframe(-2,-0.5)(2,0.5)
    \rput(0,0){#1}

}

% Sum (reference point at the center of the circle)
\def\sumsymbol{

    \pscircle(0,0){0.25}
    \rput(0,0){$+$}

}

% Analysis part of a filter bank channel (reference point at the begining of the channel)
% Parameter #1: analysis filter label
% Parameter #2: downsampling factor
\def\analysis#1#2{

    \psline{-}(0,0)(0.5,0)
    \rput(1.5,0){\filter{#1}}
    \psline{-}(2.5,0)(3,0)
    \rput(3.5,0){\downsampling{#2}}
    \psline{-}(4,0)(4.5,0)
}

% Analysis part of a filter bank channel (reference point at the begining of the channel)
% Parameter #1: analysis filter label
% Parameter #2: downsampling factor
\def\wideanalysis#1#2{

    \psline{-}(0,0)(0.5,0)
    \rput(2.5,0){\widefilter{#1}}
    \psline{-}(4.5,0)(5,0)
    \rput(5.5,0){\downsampling{#2}}
    \psline{-}(6,0)(6.5,0)
}

% Synthesis part of a filter bank channel (reference point at the begining of the channel)
% Parameter #1: synthesis filter label
% Parameter #2: upsampling factor
\def\synthesis#1#2{

    \psline{-}(0,0)(0.5,0)
    \rput(1,0){\upsampling{#2}}
    \psline{-}(1.5,0)(2,0)
    \rput(3,0){\filter{#1}}
    \psline{-}(4,0)(4.5,0)
}

% Filter bank channel (reference point at the begining of the channel)
% Parameter #1: analysis filter label
% Parameter #2: synthesis filter label
% Parameter #3: down/upsampling factor
\def\filterbankchannel#1#2#3{

    \rput(0,0){\analysis{#1}{#3}}
    \rput(4.5,0){\synthesis{#2}{#3}}

}

% Two channel filter bank (reference point at the begining of the filter bank)
% Parameter #1: lowpass analysis filter label
% Parameter #2: lowpass synthesis filter label
% Parameter #3: highpass analysis filter label
% Parameter #4: highpass synthesis filter label

\def\twochannelfilterbank#1#2#3#4{

    % Input
    \psline{*-}(0,0)(0.5,0)
    \psline{-}(0.5,-0.75)(0.5,0.75)

    % Highpass branch
    \rput(0.5,0.75){\filterbankbranch{#3}{#4}{2}}

    % Lowpass branch
    \rput(0.5,-0.75){\filterbankbranch{#1}{#2}{2}}

    % Output
    \psline{->}(9.5,0.75)(9.5,0.25)
    \rput(9.5,0){\sumsymbol}
    \psline{->}(9.5,-0.75)(9.5,-0.25)
    \psline{-*}(9.75,0)(10.25,0)

}




% Parameter #1: filter label
% Parameter #2: sampling factor
% Parameter #3: delay
\def\mybranch#1#2#3{
    \psline{-}(0,0)(0.5,0)
    \rput(1,0){\upsampling{#2}}
    \psline{-}(1.5,0)(2,0)
    \rput(2.75,0){\shortfilter{#3}}
    \psline{-}(3.5,0)(4,0)
    \rput(5,0){\filter{#1}}
    \psline{-}(6,0)(6.5,0)
    \rput(7,0){\downsampling{#2}}
    \psline{-}(7.5,0)(8,0)
}


\def\mybranchA#1#2{
    \psline{-}(-0.5,0)(0.5,0)
    \rput(1,0){\upsampling{#2}}
    \psline{-}(1.5,0)(4,0)
    \rput(5,0){\filter{#1}}
    \psline{-}(6,0)(6.5,0)
    \rput(7,0){\downsampling{#2}}
    \psline{-}(7.5,0)(8.5,0)
}


\def\mybranchB#1#2#3{
    \psline{-}(0,0)(0.5,0)
    \rput(1.5,0){\filter{#1}}
    \psline{-}(2.5,0)(3,0)
    \rput(3.5,0){\upsampling{#2}}
    \psline{-}(4,0)(4.5,0)
    \rput(5.25,0){\shortfilter{#3}}
    \psline{-}(6,0)(6.5,0)
    \rput(7,0){\downsampling{#2}}
    \psline{-}(7.5,0)(8,0)
}


\def\mybranchC#1#2{
    \psline{-}(-0.5,0)(0.5,0)
    \rput(1.5,0){\filter{#1}}
    \psline{-}(2.5,0)(3,0)
    \rput(3.5,0){\upsampling{#2}}
    \psline{-}(4,0)(6.5,0)
    \rput(7,0){\downsampling{#2}}
    \psline{-}(7.5,0)(8.5,0)
}
